3D Reconstruction of Curvilinear Structures with Stereo Matching DeepConvolutional Neural Networks

Curvilinear structures frequently appear in microscopy imaging as the object of interest. Crystallographic defects, i.e., dislocations, are one of the curvilinear structures that have been repeatedly investigated under transmission electron microscopy (TEM) and their 3D structural information is of great importance for understanding the properties of materials. 3D information of dislocations is often obtained by tomography which is a cumbersome process since it is required to acquire many images with different tilt angles and similar imaging conditions. Although, alternative stereoscopy methods lower the number of required images to two, they still require human intervention and shape priors for accurate 3D estimation. We propose a fully automated pipeline for both detection and matching of curvilinear structures in stereo pairs by utilizing deep convolutional neural networks (CNNs) without making any prior assumption on 3D shapes. In this work, we mainly focus on 3D reconstruction of dislocations from stereo pairs of TEM images.

==> figures/projections_dislocation.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}[!t]
\centering

\hfil
\begin{overpic}[width=1\hsize]{figures/proj_joint.png}
\end{overpic}
\vspace{0.5cm}
\caption{\eo{Back-projections to other views. 3D shape estimated using pairs of stereo views at 18 and 20 degree are projected back to 10 (a), 14 (b), 16 (c) degree views.}} 
%Projections to other views. 3D shape estimated from 18 and 20 degree views projected back to 10 (a), 14 (b), 16 (c) degree views.}.
\EO{Please: 1-add scale-bar, 2- Flip the images in the upper row, 3- crop the upper row images so that they include only dislocations with the backprojected points. I think instead of back projecting the points, we should first convert the points to lines (after removing the outliers) and backproject the lines on the images, and maybe show on the image both segmented dislocation (traced line) and back-projected lines.}
\label{fig:projections}
\end{figure*}



==> figures/stereo_matching_network.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[!t]
\centering
\begin{overpic}[width=1.0\hsize]{figures/stereo_matching_network.png}
\end{overpic}
\vspace{0.5cm}
\caption{Stereo Matching Network Architecture. Layers with learnable parameters are shown in blue. }
\label{fig:stereonet}
\end{figure}

==> tex/conclusion.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\section{Conclusion}

Stereo-vision remains to be an acceptable alternative 3D reconstruction approach for curvilinear structures especially when acquiring large number of images is costly in terms of time and manual effort. Moreover, thanks to the recent advancements in deep neural networks, detection and matching tasks now may be combined in one neural network architecture and learned jointly. In this paper, we have therefore proposed a network architecture designed for matching curvilinear structures that delivers good performance in a wide variety of microscopy images while automatizing the process. We also introduced a novel loss term, \textit{variance loss}, which increased our network's localization capability. 

